The Surprising Effectiveness of Diffusion Models for Optical Flow and Monocular Depth Estimation

Denoising diffusion probabilistic models have transformed image generation with their impressive fidelity and diversity. We show that they also excel in estimating optical flow and monocular depth, surprisingly, without task-specific architectures and loss functions that are predominant for these tasks. Compared to the point estimates of conventional regression-based methods, diffusion models also enable Monte Carlo inference, e.g., capturing uncertainty and ambiguity in flow and depth. With self-supervised pre-training, the combined use of synthetic and real data for supervised training, and technical innovations (infilling and step-unrolled denoising diffusion training) to handle noisy-incomplete training data, and a simple form of coarse-to-fine refinement, one can train state-of-the-art diffusion models for depth and optical flow estimation. Extensive experiments focus on quantitative performance against benchmarks, ablations, and the model's ability to capture uncertainty and multimodality, and impute missing values. Our model, DDVM (Denoising Diffusion Vision Model), obtains a state-of-the-art relative depth error of 0.074 on the indoor NYU benchmark and an Fl-all outlier rate of 3.26\% on the KITTI optical flow benchmark, about 25\% better than the best published method. For an overview see https://diffusion-vision.github.io.

==> images_tex/image_flow_raft_comp_rebuttal.tex <==

\begin{figure*}[!h]
    \centering
    \scriptsize
    \setlength\tabcolsep{1pt} % default value: 6pt
    \newcommand{\Figwidth}{0.245\linewidth}
    \begin{tabular}{cccc}
      First frame & Ground Truth & RAFT & \textbf{Ours} \\
    \includegraphics[trim={0 40 0 80},clip,width=\Figwidth]{images/flow_raft_pretrain_comparisons/sintelfinal_0017/frame0.jpg} &
    \includegraphics[trim={0 40 0 80},clip,width=\Figwidth]{images/flow_raft_pretrain_comparisons/sintelfinal_0017/gt.jpg} &
    \includegraphics[trim={0 40 0 80},clip,width=\Figwidth]{images/flow_raft_pretrain_comparisons/sintelfinal_0017/pred_raft.jpg} &
    \includegraphics[trim={0 40 0 80},clip,width=\Figwidth]{images/flow_raft_pretrain_comparisons/sintelfinal_0017/pred_diff.jpg} \\
    \includegraphics[trim={0 120 0 0},clip,width=\Figwidth]{images/flow_raft_pretrain_comparisons/kitti_0087/frame0.jpg} &
    \includegraphics[trim={0 120 0 0},clip,width=\Figwidth]{images/flow_raft_pretrain_comparisons/kitti_0087/gt.jpg} &
    \includegraphics[trim={0 120 0 0},clip,width=\Figwidth]{images/flow_raft_pretrain_comparisons/kitti_0087/pred_raft.jpg} &
    \includegraphics[trim={0 120 0 0},clip,width=\Figwidth]{images/flow_raft_pretrain_comparisons/kitti_0087/pred_diff.jpg} \\
    \end{tabular}
        \vspace*{-0.1cm}
	\caption{\textbf{Visual results comparing RAFT with our method after pretraining}. Note that our method does much better on fine details and ambiguous regions.}
    \label{fig:flow_raft_pretrain_comparison}
    \vspace{-1em}
\end{figure*}


==> not_used/result_flow_dataset_ablation.tex <==
\begin{table}

\centering
\footnotesize

\caption{Zero-shot results for different dataset mixtures for the Sintel and KITTI datasets.}
\label{tab:flow-dataset-ablation}
\vspaceaftercaption

\begin{tabular}{lccccc}
\toprule
Dataset & Sintel.clean & Sintel.final & KITTI & KITTI Fl-all\\ 
 \hline
 AF & 2.04 & 2.55 & 4.47 & 16.59\% \\
 AF$\rightarrow$AF+FT & 1.48 & 2.22 & 3.71 & 14.07\% \\
 AF$\rightarrow$AF+FT+KU & 1.33 &  2.04 &  2.82 & 9.27\% \\
AF$\rightarrow$AF+FT+KU+TA &  \textbf{1.24} & \textbf{2.00} & \textbf{2.19} & \textbf{7.58\%} \\
\bottomrule
\end{tabular}

\end{table}

==> not_used/table_flow_finetuning.tex <==
\begin{table}[t]
\centering
\scriptsize
    \caption{{\bf Optical flow finetuning evaluation} on public benchmark datasets (AEPE$\downarrow$ for Sintel and Fl-all$\downarrow$ for KITTI). 
    \textbf{Bold} indicates the best and \underline{underline} the \nth{2}-best.
    $^{\S}$ uses extra datasets (AutoFlow and VIPER) on top of defaults (FlyingThings, HD1K, KITTI, and Sintel). $^*$uses warm start on Sintel.
    }
    \label{tab:flow_benchmark}

    \setlength\tabcolsep{2.15pt}
    \begin{tabularx}{0.4\linewidth}{X @{\hskip 1em} cccc}
    \toprule
    Method & Sintel.clean & Sintel.final & KITTI \\ \midrule
    % PWC-Net~\cite{sun2018pwc}  &  3.86 & 5.13  & 9.60\% & 30ms$^*$\\
    % PWC-Net+~\cite{sun2019models} &  3.45 & 4.60  & 7.72\% & 30ms$^*$ \\
    % PWC-Net (Ours)  & 2.37 & 3.79  & 5.54\% & 21ms\\ \hline 
    % PWC-Net-it  & 2.31 & 3.69  & 5.54\% & \textbf{21ms}\\ %\hline 
    % IRR-PWC~\cite{hur2019iterative} & 3.84 & 4.58 & 7.65\%  & 180ms$^*$\\ %
    % IRR-PWC-it  &2.19 & 3.55 & 5.73\% & \underline{25ms} \\  %\hline
    % Modified IRR-PWC & TO & ADD \\ \hline
    % RAFT v1~\cite{teed2020raft} & 2.77 & 3.61 & 6.30\% \\
    % RAFT-A~\cite{sun2021autoflow} & 2.01 & {3.14} &  {4.78}\% & 107ms\\
    % GMFlow \citep{xu2022gmflow} & 1.74 & 2.90 & 9.32\% \\ % KITTI number too bad
    % GMA \citep{jiang2021learning}$^*$ & 1.39 & 2.47 & 5.15\% \\ 
    % RAFT~\citep{teed2020raft} & 1.94 &  3.18 & 5.10\% \\ % 200
    % RAFT~\citep{teed2020raft}$^*$ & 1.61 &  2.86 & - \\ % 200
    % AGFlow~\citep{luo2022learning}$^*$ & 1.43 & 2.47 & 4.89\% \\
    % MS$\_$RAFT \citep{jahedi2022multi} & 1.37 & 2.67 & 4.88\% \\
    SKFlow \citep{sunskflow}$^*$ & \underline{1.30} & \underline{2.26} & 4.84\% \\ 
    CRAFT \citep{sui2022craft}$^*$ & {1.44} & 2.42 & 4.79\% \\
    FlowFormer \citep{huang2022flowformer} & \textbf{1.14} & \textbf{2.18} & 4.68\% \\ 
    % SeparableFlow \citep{zhang2021separable} & 1.50 & 2.67 & 4.64\% \\ 
    RAFT-OCTC~\citep{jeong2022imposing}$^{*}$ & 1.51 &2.57 & 4.33\% \\
    RAFT-it~\citep{sun2022disentangling}$^{\S}$ & 1.55 & 2.90 & \underline{4.31\%} \\
    \textbf{\ours}$^{\S}$ & 1.75 & 2.48 & \textbf{3.26\%} \\ 
    \hline
    
    % \hline HD$^3$\cite{yin2019hierarchical} & 4.79 & 4.67 & 6.55\% & 100ms$^*$  \\
    % VCN~\cite{yang2018segstereo} & 2.81 & 4.40 & 6.30\%  &180ms$^*$\\
    % Mask-FlowNet~\cite{zhao2020maskflownet} & 2.52	 & 4.14 &	6.11\%  & 60ms$^*$ \\
    % DICL~\cite{wang2020displacement} & 2.12 & 3.44 &  6.31\% & - \\
    % Flow1D~\cite{xu2021flow1d} & 2.24 & 3.81 & 6.27\% & 79ms$^*$ \\ 
    % RAFT+AOIR~\cite{mehl2021anisotropic} &1.85 & 3.17 & 5.07\% & 10$^4$ms$^*$\\
    % CSFlow~\cite{shi2022csflow} & 1.63 & 3.03 & 5.00\% & 200ms$^*$ \\
    % SeparableFlow~\cite{zhang2021separable} & \textbf{1.50} & \textbf{2.67} & \underline{4.51\%} & 250ms$^*$ \\ 
    \end{tabularx}
\end{table}




% \begin{table}[t]
% \centering
% \begin{minipage}[t]{.4\textwidth}
%     \centering
%     \scriptsize

% \end{minipage} \;
% \begin{minipage}[t]{.57\textwidth}
%     \vspace{0.8em}
%     \scriptsize
%     \centering
    

% \end{minipage}

% \end{table}

% \begin{table}[t]
% \centering
% % \begin{adjustbox}{width=0.8\textwidth}

% \vspaceaftercaption

% % \aftertable
% \end{table}




% \begin{table}[t]
% \centering
% % \begin{adjustbox}{width=0.8\textwidth}
% \scriptsize
% \caption{Optical flow {\bf finetuning evaluation} on public benchmark datasets (AEPE$\downarrow$ for Sintel and Fl-all$\downarrow$ for KITTI). 
%  \textbf{Bold} indicates the best and \underline{underline} the \nth{2}-best.
% \srbs{Should we discuss why (we think) we are worse on Sintel and much better on KITTI in text? In short, sintel test and train distributions are very different whereas kitti train and test are similar. So cost volume based approaches are expected to perform better as they should be more robust to OOD.} \ds{We may remove Robust from our title.} \ds{Among methods without warm start, only FlowFormer is significantly better, probably due to attention on the cost volume.}
% $^{\S}$ uses extra datasets (AutoFlow and ViPER) on top of defaults (FlyingThings, HD1K, KITTI, and Sintel). $^*$ uses warm start on Sintel.}
% \vspaceaftercaption
% \begin{tabular}{lcccc}
% \toprule
% Method & Sintel.clean & Sintel.final & KITTI \\ \midrule
% % PWC-Net~\cite{sun2018pwc}  &  3.86 & 5.13  & 9.60\% & 30ms$^*$\\
% % PWC-Net+~\cite{sun2019models} &  3.45 & 4.60  & 7.72\% & 30ms$^*$ \\
% % PWC-Net (Ours)  & 2.37 & 3.79  & 5.54\% & 21ms\\ \hline 
% % PWC-Net-it  & 2.31 & 3.69  & 5.54\% & \textbf{21ms}\\ %\hline 
% % IRR-PWC~\cite{hur2019iterative} & 3.84 & 4.58 & 7.65\%  & 180ms$^*$\\ %
% % IRR-PWC-it  &2.19 & 3.55 & 5.73\% & \underline{25ms} \\  %\hline
% % Modified IRR-PWC & TO & ADD \\ \hline
% % RAFT v1~\cite{teed2020raft} & 2.77 & 3.61 & 6.30\% \\
% % RAFT-A~\cite{sun2021autoflow} & 2.01 & {3.14} &  {4.78}\% & 107ms\\
% % GMFlow \citep{xu2022gmflow} & 1.74 & 2.90 & 9.32\% \\ % KITTI number too bad
% GMA \citep{jiang2021learning}$^*$ & 1.39 & 2.47 & 5.15\% \\ 
% RAFT~\citep{teed2020raft} & 1.94 &  3.18 & 5.10\% \\ % 200
% RAFT~\citep{teed2020raft}$^*$ & 1.61 &  2.86 & - \\ % 200
% AGFlow~\citep{luo2022learning}$^*$ & 1.43 & 2.47 & 4.89\% \\
% MS$\_$RAFT \citep{jahedi2022multi} & 1.37 & 2.67 & 4.88\% \\
% SKFlow \citep{sunskflow}$^*$ & \underline{1.30} & \underline{2.26} & 4.84\% \\ 
% CRAFT \citep{sui2022craft}$^*$ & {1.44} & 2.42 & 4.79\% \\
% FlowFormer \citep{huang2022flowformer} & \textbf{1.14} & \textbf{2.18} & 4.68\% \\ 
% SeparableFlow \citep{zhang2021separable} & 1.50 & 2.67 & 4.64\% \\ 
% RAFT-OCTC~\citep{jeong2022imposing}$^{*}$ & 1.51 &2.57 & 4.33\% \\
% RAFT-it~\citep{sun2022disentangling}$^{\S}$ & 1.55 & 2.90 & \underline{4.31\%} \\
% \textbf{\ours}$^{\S}$ & 1.75 & 2.48 & \textbf{3.26\%} \\ 
% \hline

% % \hline HD$^3$\cite{yin2019hierarchical} & 4.79 & 4.67 & 6.55\% & 100ms$^*$  \\
% % VCN~\cite{yang2018segstereo} & 2.81 & 4.40 & 6.30\%  &180ms$^*$\\
% % Mask-FlowNet~\cite{zhao2020maskflownet} & 2.52	 & 4.14 &	6.11\%  & 60ms$^*$ \\
% % DICL~\cite{wang2020displacement} & 2.12 & 3.44 &  6.31\% & - \\
% % Flow1D~\cite{xu2021flow1d} & 2.24 & 3.81 & 6.27\% & 79ms$^*$ \\ 
% % RAFT+AOIR~\cite{mehl2021anisotropic} &1.85 & 3.17 & 5.07\% & 10$^4$ms$^*$\\
% % CSFlow~\cite{shi2022csflow} & 1.63 & 3.03 & 5.00\% & 200ms$^*$ \\
% % SeparableFlow~\cite{zhang2021separable} & \textbf{1.50} & \textbf{2.67} & \underline{4.51\%} & 250ms$^*$ \\ 
% \end{tabular}
% % \end{adjustbox}
% \label{tab:flow_benchmark}
% % \aftertable
% \end{table}


==> not_used/table_flow_zero_shot.tex <==
\begin{table}[t]
\centering
\scriptsize

\caption{\textbf{Zero-shot results on Sintel and KITTI}. We provide a new RAFT baseline using our proposed pre-training mixture and substantially improve the accuracy over the original. Our diffusion model outperforms even this much stronger baseline and achieves state-of-the-art zero-shot results on challenging Sintel.final and KITTI.}
\label{tab:flow-pretrain-results}

\setlength\tabcolsep{1.15pt}
    \begin{tabular}{l l @{\hskip 1em} cccc}
    \toprule
    \multirow{2}{*}{Model} &  \multirow{2}{*}{Dataset} & Sintel.clean & Sintel.final & \multicolumn{2}{c}{KITTI} \\ 
    \cmidrule(lr){3-4} \cmidrule(lr){5-6}
     &    & \multicolumn{2}{c}{AEPE} & AEPE & Fl-all \\ 
     \midrule
    FlowFormer &  Chairs~$\!\rightarrow\!$~Things  & \textbf{1.01} & 2.40 & 4.09 &  14.72\% \\  %
    RAFT & Chairs~$\!\rightarrow\!$~Things & {1.68}	&2.80	&5.92 & -\\
    % FlowFormer++  &  Chairs~$\!\rightarrow\!$~Things \\  # unpublished
    % \hline \multirow{3}{*}{PWC-Net} & FlyingChairs &  3.27	& 4.42 & 11.43 & -\\ 
    % & Chairs~$\!\rightarrow\!$~Things &	2.39	& 3.90 & 9.81 & -\\
    % & AutoFlow (3.2M) & {\pwcsintelclean} &	{\pwcsintelfinal} & {\pwckitti} & -\\ 
    % & AutoFlow (6.2M) & 2.10 &	2.81  & 5.55 & - \\ %& 16.29\%
    \midrule 
    % \multirow{3}{*}{ RAFT}
    % & FlyingChairs &2.27	&3.76	&7.63 & -	\\ 
    Perceiver IO & AutoFlow (AF) & 1.81 & 2.42 &  4.98 & -\\ 
    % & AutoFlow (0.8M)  & {\raftsintelclean} &	{\raftsintelfinal} & {\raftkitti} & -\\ 
    RAFT & AutoFlow   & 1.74	&2.41	&4.18  &   13.41\% \\ 
    \midrule
    {RAFT (ours)}
    & AF$\rightarrow$AF+FT+KU+TA & 1.27 &	2.28 &	2.71 & 9.16\% \\
    % \hline\multirow{1}{*}{ \ours } & AF \\
    \midrule
    \multirow{4}{*}{\textbf{Ours}} &AF & 2.04 & 2.55 & 4.47 & 16.59\% \\
     &AF$\rightarrow$AF+FT & 1.48 & 2.22 & 3.71 & 14.07\% \\
     &AF$\rightarrow$AF+FT+KU & 1.33 &  2.04 &  2.82 & 9.27\% \\
    &AF$\rightarrow$AF+FT+KU+TA &  {1.24} & \textbf{2.00} & \textbf{2.19} & \textbf{7.58\%} \\
    % \textbf{\ours} & AF$\rightarrow$AF+FT+KU+TA &  1.24 & \textbf{2.00} & \textbf{2.19} & \textbf{7.58}\% \\
    \bottomrule
    \end{tabular}
\end{table}



% \begin{table}[t]
% \centering
% \scriptsize

% \caption{\textbf{Zero-shot results on Sintel and KITTI}. We provide a new RAFT baseline using our proposed pre-training mixture and substantially improve the accuracy over the original. Our diffusion model outperforms even this much stronger baseline and achieves state-of-the-art zero-shot results on challenging Sintel.final and KITTI.}
% \label{tab:flow-pretrain-results}

% \setlength\tabcolsep{1.15pt}
%     \begin{tabularx}{0.6\linewidth}{X @{\hskip 0.5em} l @{\hskip 1em} cccc}
%     \toprule
%     \multirow{2}{*}{Model} &  \multirow{2}{*}{Dataset} & Sintel.clean & Sintel.final & \multicolumn{2}{c}{KITTI} \\ 
%     \cmidrule(lr){3-4} \cmidrule(lr){5-6}
%      &    & \multicolumn{2}{c}{AEPE} & AEPE & Fl-all \\ 
%      \midrule
%     FlowFormer &  Chairs~$\!\rightarrow\!$~Things  & \textbf{1.01} & 2.40 & 4.09 &  14.72\% \\  %
%     RAFT & Chairs~$\!\rightarrow\!$~Things & {1.68}	&2.80	&5.92 & -\\
%     % FlowFormer++  &  Chairs~$\!\rightarrow\!$~Things \\  # unpublished
%     % \hline \multirow{3}{*}{PWC-Net} & FlyingChairs &  3.27	& 4.42 & 11.43 & -\\ 
%     % & Chairs~$\!\rightarrow\!$~Things &	2.39	& 3.90 & 9.81 & -\\
%     % & AutoFlow (3.2M) & {\pwcsintelclean} &	{\pwcsintelfinal} & {\pwckitti} & -\\ 
%     % & AutoFlow (6.2M) & 2.10 &	2.81  & 5.55 & - \\ %& 16.29\%
%     \midrule 
%     % \multirow{3}{*}{ RAFT}
%     % & FlyingChairs &2.27	&3.76	&7.63 & -	\\ 
%     Perceiver IO & AutoFlow (AF) & 1.81 & 2.42 &  4.98 & -\\ 
%     % & AutoFlow (0.8M)  & {\raftsintelclean} &	{\raftsintelfinal} & {\raftkitti} & -\\ 
%     RAFT & AutoFlow   & 1.74	&2.41	&4.18  &   13.41\% \\ 
%     \midrule
%     {RAFT (ours)}
%     & AF$\rightarrow$AF+FT+KU+TA & 1.27 &	2.28 &	2.71 & 9.16\% \\
%     % \hline\multirow{1}{*}{ \ours } & AF \\
%     \midrule
%     \multirow{4}{*}{\textbf{Ours}} &AF & 2.04 & 2.55 & 4.47 & 16.59\% \\
%      &AF$\rightarrow$AF+FT & 1.48 & 2.22 & 3.71 & 14.07\% \\
%      &AF$\rightarrow$AF+FT+KU & 1.33 &  2.04 &  2.82 & 9.27\% \\
%     &AF$\rightarrow$AF+FT+KU+TA &  {1.24} & \textbf{2.00} & \textbf{2.19} & \textbf{7.58\%} \\
%     % \textbf{\ours} & AF$\rightarrow$AF+FT+KU+TA &  1.24 & \textbf{2.00} & \textbf{2.19} & \textbf{7.58}\% \\
%     \bottomrule
%     \end{tabularx}
% \end{table}





% \begin{table}
% \centering
% % \begin{adjustbox}{width=1.0\textwidth}
% \scriptsize

% \vspaceaftercaption

% % \end{adjustbox}
% % \end{center}
% \end{table}




% \begin{table}
% \centering
% % \begin{adjustbox}{width=1.0\textwidth}
% \scriptsize
% \caption{\textbf{Zero-shot results on Sintel and KITTI}: We provide a new RAFT baseline using our proposed pre-training mixture and substantially improve the accuracy over the original. Our diffusion model outperforms even this much stronger baseline and achieves state-of-the-art zero-shot results on challenging Sintel.final and KITTI.}
% \label{tab:flow-pretrain-results}
% \vspaceaftercaption
% \begin{tabular}{llcccc} 
% \toprule
% \multirow{2}{*}{Model} &  \multirow{2}{*}{Dataset} & Sintel.clean & Sintel.final & \multicolumn{2}{c}{KITTI} \\ 
%  &    & \multicolumn{2}{c}{AEPE} & AEPE & Fl-all \\ 
%  \midrule
% FlowFormer &  Chairs~$\!\rightarrow\!$~Things  & \textbf{1.01} & 2.40 & 4.09 &  14.72\% \\  %
% RAFT & Chairs~$\!\rightarrow\!$~Things & {1.68}	&2.80	&5.92 & -\\
% % FlowFormer++  &  Chairs~$\!\rightarrow\!$~Things \\  # unpublished
% % \hline \multirow{3}{*}{PWC-Net} & FlyingChairs &  3.27	& 4.42 & 11.43 & -\\ 
% % & Chairs~$\!\rightarrow\!$~Things &	2.39	& 3.90 & 9.81 & -\\
% % & AutoFlow (3.2M) & {\pwcsintelclean} &	{\pwcsintelfinal} & {\pwckitti} & -\\ 
% % & AutoFlow (6.2M) & 2.10 &	2.81  & 5.55 & - \\ %& 16.29\%
% \midrule 
% % \multirow{3}{*}{ RAFT}
% % & FlyingChairs &2.27	&3.76	&7.63 & -	\\ 
% Perceiver IO & AutoFlow (AF) & 1.81 & 2.42 &  4.98 & -\\ 
% % & AutoFlow (0.8M)  & {\raftsintelclean} &	{\raftsintelfinal} & {\raftkitti} & -\\ 
% RAFT & AutoFlow   & 1.74	&2.41	&4.18  &   13.41\% \\ 
% \midrule
% {RAFT (ours)}
% & AF$\rightarrow$AF+FT+KU+TA & 1.27 &	2.28 &	2.71 & 9.16\% \\
% % \hline\multirow{1}{*}{ \ours } & AF \\
% \midrule
% \multirow{4}{*}{\textbf{Ours}} &AF & 2.04 & 2.55 & 4.47 & 16.59\% \\
%  &AF$\rightarrow$AF+FT & 1.48 & 2.22 & 3.71 & 14.07\% \\
%  &AF$\rightarrow$AF+FT+KU & 1.33 &  2.04 &  2.82 & 9.27\% \\
% &AF$\rightarrow$AF+FT+KU+TA &  {1.24} & \textbf{2.00} & \textbf{2.19} & \textbf{7.58\%} \\
% % \textbf{\ours} & AF$\rightarrow$AF+FT+KU+TA &  1.24 & \textbf{2.00} & \textbf{2.19} & \textbf{7.58}\% \\
% \bottomrule
% \end{tabular}
% % \end{adjustbox}
% % \end{center}
% \end{table}
